MPClan: Protocol Suite for Privacy-Conscious Computations

The growing volumes of data being collected and its analysis to provide better services are creating worries about digital privacy. To address privacy concerns and give practical solutions, the literature has relied on secure multiparty computation. However, recent research has mostly focused on the small-party honest-majority setting of up to four parties, noting efficiency concerns. In this work, we extend the strategies to support a larger number of participants in an honest-majority setting with efficiency at the center stage. Cast in the preprocessing paradigm, our semi-honest protocol improves the online complexity of the decade-old state-of-the-art protocol of Damg\aa rd and Nielson (CRYPTO'07). In addition to having an improved online communication cost, we can shut down almost half of the parties in the online phase, thereby saving up to 50% in the system's operational costs. Our maliciously secure protocol also enjoys similar benefits and requires only half of the parties, except for one-time verification, towards the end. To showcase the practicality of the designed protocols, we benchmark popular applications such as deep neural networks, graph neural networks, genome sequence matching, and biometric matching using prototype implementations. Our improved protocols aid in bringing up to 60-80% savings in monetary cost over prior work.

==> Main_Conclusion.tex <==
We design an efficient semi-honest protocol for the multiparty setting in the preprocessing model with an improved online phase communication complexity compared to the state-of-the-art protocol of DN07. 
%
We further design an efficient maliciously secure protocol with minimal overhead in the online phase. Our protocols require active participation from only half of the parties (for most of the computation, in the malicious setting) in the online phase . 
%
We benchmark, for the first time in the multiparty setting, applications such as deep NN, GNN, SSQ and biometric matching, and observe significant improvements over DN07. 
%
We leave the problem of optimizing the complexity of the building blocks as an interesting open question. Another interesting direction is to explore the efficiency improvements contributed by our building blocks in algorithms such as Decision Tress, k-Means Clustering, Binarized Neural Networks etc.




==> symbols/symbols_4pc_SWIFT.tex <==
%--------------------------------------------------------------
%FourPC Variables and Notations
%--------------------------------------------------------------
%\newcommand{\A}{\mathsf{A}}
%\newcommand{\B}{\mathsf{B}}
\newcommand{\R}{\mathsf{R}}
%\newcommand{\ve}{\mathsf{e}}

%Terms
\newcommand{\JmpF}{\ensuremath{\mathsf{jmp4}}}
\newcommand{\Gammaxdy}{\ensuremath{\Gamma_{\vecX \band \vecY}}}

%JmpF primitive
\newcommand{\jsendf}{\ensuremath{\mathsf{jmp4\mbox{-}send}}}

\newcommand{\PlSet}[1]{\ensuremath{\Phi_{#1}}}
%\newcommand{\PlSet}[1]{\ensuremath{\rho_{#1}}}

%--------------------------------------------------------------
%FourPC Protocols
%--------------------------------------------------------------
\newcommand{\piJmpF}{\ensuremath{\Pi_{\mathsf{jmp4}}}}
%\newcommand{\pifinput}{\ensuremath{\Pi_{\mathsf{sh4}}}}
\newcommand{\pifinputS}{\ensuremath{\Pi_{\mathsf{sh}^{\SOC}}}}
%\newcommand{\pifmul}{\ensuremath{\Pi_{\mathsf{mult4}}}}
\newcommand{\pifrec}{\ensuremath{\Pi_{\mathsf{rec4}}}}
\newcommand{\pifrecS}{\ensuremath{\Pi_{\mathsf{rec}}^{\SOC}}}
\newcommand{\pifjsh}{\ensuremath{\Pi_{\mathsf{jsh4}}}}
\newcommand{\pifbitext}{\ensuremath{\Pi_{\mathsf{bitext4}}}}
\newcommand{\pifbita}{\ensuremath{\Pi_{\mathsf{bit2A4}}}}
\newcommand{\pifdotp}{\ensuremath{\Pi_{\mathsf{dotp4}}}}
\newcommand{\piftrgen}{\ensuremath{\Pi_{\mathsf{trgen4}}}}
\newcommand{\pifdotpt}{\ensuremath{\Pi_{\mathsf{dotpt4}}}}
\newcommand{\piBitInjF}{\ensuremath{\Pi_{\mathsf{bitinj4}}}}
%\newcommand{\pifsgrsh}{\ensuremath{\Pi_{\mathsf{ash4}}}}

%--------------------------------------------------------------
%FourPC Functionalities
%--------------------------------------------------------------
\newcommand{\Funcf}{\ensuremath{\mathcal{F}_{\mathsf{4PC}}}}
\newcommand{\FSETUPf}{\ensuremath{\mathcal{F}_{\mathsf{setup4}}}}
\newcommand{\FJmpF}{\ensuremath{\mathcal{F}_{\mathsf{jmp4}}}}
\newcommand{\FShF}{\ensuremath{\mathcal{F}_{\mathsf{sh4}}}}
\newcommand{\FMulF}{\ensuremath{\mathcal{F}_{\mathsf{mult4}}}}
\newcommand{\FReconF}{\ensuremath{\mathcal{F}_{\mathsf{rec4}}}}
\newcommand{\FJshF}{\ensuremath{\mathcal{F}_{\mathsf{jsh4}}}}
\newcommand{\FBitextF}{\ensuremath{\mathcal{F}_{\mathsf{bitext4}}}}
\newcommand{\FBitaF}{\ensuremath{\mathcal{F}_{\mathsf{bit2A4}}}}
\newcommand{\FDotpF}{\ensuremath{\mathcal{F}_{\mathsf{dotp4}}}}
\newcommand{\FTrgenF}{\ensuremath{\mathcal{F}_{\mathsf{trgen4}}}}
\newcommand{\FBitInjF}{\ensuremath{\mathcal{F}_{\mathsf{bitinj4}}}}
